Let Trajectories Speak Out the Traffic Bottlenecks

Traffic bottlenecks are a set of road segments that have an unacceptable level of traffic caused by a poor balance between road capacity and traffic volume. A huge volume of trajectory data which captures real-time traffic conditions in road networks provides promising new opportunities to identify the traffic bottlenecks. In this paper, we define this problem as trajectory-driven traffic bottleneck identification: Given a road network R, a trajectory database T , find a representative set of seed edges of size K of traffic bottlenecks that influence the highest number of road segments not in the seed set. We show that this problem is NP-hard and propose a framework to find the traffic bottlenecks as follows. First, a traffic spread model is defined which represents changes in traffic volume for each road segment over time. Then, the traffic diffusion probability between two connected segments and the residual ratio of traffic volume for each segment can be computed using historical trajectory data. We then propose two different algorithmic approaches to solve the problem. The first one is a best-first algorithm BF, with an approximation ratio of 1-1/e. To further accelerate the identification process in larger datasets, we also propose a sampling-based greedy algorithm SG. Finally, comprehensive experiments using three different datasets compare and contrast various solutions, and provide insights into important efficiency and effectiveness trade-offs among the respective methods.

==> fig-exp3.tex <==
\begin{figure*}[t]
	\centering
	\subfigure[Runtime (Grid)]{
		\label{fig:cd:runtime:grid}
		\includegraphics[width=\graphscaleHalf\textwidth]{figure/exp/chengdu_time_grid.pdf}
	}
	\subfigure[Influence Score (Grid)]{
		\label{fig:cd:influ:grid}
		\includegraphics[width=\graphscaleHalf\textwidth]{figure/exp/chengdu_influ_grid.pdf}
	}
	%\hspace{4ex}
	\subfigure[Runtime (KMeans)]{
		\label{fig:cd:runtime:kmeans}
		\includegraphics[width=\graphscaleHalf\textwidth]{figure/exp/chengdu_time_kmeans.pdf}
	}
	\subfigure[Influence Score (KMeans)]{
		\label{fig:cd:influ:kmeans}
		\includegraphics[width=\graphscaleHalf\textwidth]{figure/exp/chengdu_influ_kmeans.pdf}
	}
	\caption{Performance comparison of partition-based methods in \chengdu dataset.}
	\label{fig:cd:patition}
	\vspace{-2ex}
\end{figure*}


\begin{figure*}[h]
	\centering
	\subfigure[Runtime (Grid)]{
		\label{fig:xa:runtime:grid}
		\includegraphics[width=\graphscaleHalf\textwidth]{figure/exp/xian_time_grid.pdf}
	}
	\subfigure[Influence Score (Grid)]{
		\label{fig:xa:influ:grid}
		\includegraphics[width=\graphscaleHalf\textwidth]{figure/exp/xian_influ_grid.pdf}
	}
	%\hspace{4ex}
	\subfigure[Runtime (KMeans)]{
		\label{fig:xa:runtime:kmeans}
		\includegraphics[width=\graphscaleHalf\textwidth]{figure/exp/xian_time_kmeans.pdf}
	}
	\subfigure[Influence Score (KMeans)]{
		\label{fig:xa:influ:kmeans}
		\includegraphics[width=\graphscaleHalf\textwidth]{figure/exp/xian_influ_kmeans.pdf}
	}
	\caption{Performance comparison of partition-based methods in \xian dataset.}
	\label{fig:xa:patition}
	\vspace{-2ex}
\end{figure*}

==> sec3-baseline.tex <==
\section{Our Approach}\label{sec-approach}
In this section, we propose xx approximation methods with performance guarantees to solve the problem.
\subsection{Greedy Algorithm}
The greedy algorithm iteratively selects an edge $e$ into a seed set \seedSet if $e$ provides the maximum marginal gain to the total incremental influence score $\Phi(S)$ w.r.t. \seedSet (i.e., Eq. \ref{equ-obj}).
The greedy algorithm is shown in Algorithm \ref{alg-g}, which guarantees an approximation ratio of $(1-1/e)$.
\hui{the DFS can be further explained.}
\input{alg-g.tex}

\myparagraph{Time complexity}
The total time complexity is $K|E|O(|V|+|E|)$, where $\mathsf{DFS}$ spends $O(|V+E|)$.
%If the traffic diffusion has one iteration, then the influence function will have the monotonicity and submodularity properties.

\begin{lemma}
	\label{lemma-mono}
	(Monotonicity) Let \seedSet and \seedSetprime be two sets of seed edges, and $\seedSet \subseteq \seedSetprime$. Then we have:
	\begin{equation}
	\Phi(\seedSet) \leq \Phi(\seedSetprime)
	\end{equation}
\end{lemma}
\begin{proof}
	Since $\seedSet \subseteq \seedSetprime$, we have $I(\seedSetprime)=I(\seedSet) \cup I(\seedSetprime-\seedSet)$, then $I(\seedSet) \subseteq I(\seedSetprime)$. Therefore, $\Phi(\seedSetprime)=\sum_{e \in I(\seedSetprime)\cap f(e) \geq \flowPara}^{}\sigma(e)$ $\geq \sum_{e \in I(\seedSet)\cap f(e) \geq \flowPara}^{}$ $\sigma(e)= \Phi(\seedSet)$. 
\end{proof}

\begin{lemma}
	\label{lemma-sub}
	(Submodularity) Let \seedSet and \seedSetprime be two sets of seed edges, and $\seedSet \subseteq \seedSetprime$. Assume that \seed is a newly inserted edge, we have:
	\begin{equation}
	\Phi(\seedSet \cup \{\seed\}) - \Phi(\seedSet) \geq \Phi(\seedSetprime \cup \{\seed\}) - \Phi(\seedSetprime)
	\end{equation}
\end{lemma}
\begin{proof}
	Considering the different relationships between $I(\seedSet)$ and $I(\seed)$, we analyze the following cases to support the proof.
	
	\textbf{Case 1.}
	If $I(\{\seed\}) \subseteq I(\seedSet)$, then $I(\{\seed\}) \subseteq I(\seedSetprime)$. Thus $\Phi(\seedSet \cup \{\seed\}) - \Phi(\seedSet)$ = $\Phi(\seedSet) - \Phi(\seedSet) = 0$. Similarly, $\Phi(\seedSetprime \cup \{\seed\}) - \Phi(\seedSetprime)$ = $\Phi(\seedSetprime) - \Phi(\seedSetprime) = 0$. 
	
	\textbf{Case 2.}
	If $I(\{\seed\}) \cap I(\seedSet) = \emptyset$, then $I(\{\seed\}) \cap I(\seedSetprime) = \emptyset$. Then $\Phi(\seedSet \cup \{\seed\}) - \Phi(\seedSet)$ = $\Phi(\seedSet) + \Phi(\{\seed\})- \Phi(\seedSet)=\Phi(\{\seed\})$. As such, $\Phi(\seedSetprime \cup \{\seed\}) - \Phi(\seedSetprime) = \Phi(\{\seed\})$.
	
	\textbf{Case 3.}
	If $I(\{\seed\}) \cap I(\seedSet) \neq \emptyset$, we assume that $A=I(\{\seed\})-I(\{\seed\}) \cap I(\seedSet)$, then $\Phi(\seedSet \cup \{\seed\}) - \Phi(\seedSet) = \sum_{e \in A \cap f(e) \geq \flowPara}^{}\sigma(e)$. We also assume that $A^\prime=I(\{\seed\})-I(\{\seed\}) \cap I(\seedSetprime)$, then $\Phi(\seedSetprime \cup \{\seed\}) - \Phi(\seedSetprime) = \sum_{e \in A^\prime \cap f(e) \geq \flowPara}^{}\sigma(e)$. Note that $A^\prime \subseteq A$, thus we can easily obtain that $\sum_{e \in A \cap f(e) \geq \flowPara}^{}\sigma(e) \geq \sum_{e \in A^\prime \cap f(e) \geq \flowPara}^{}\sigma(e)$ based on the monotonicity property in Lemma \ref{lemma-mono}. Thus $\Phi(\seedSet \cup \{\seed\}) - \Phi(\seedSet) \geq \Phi(\seedSetprime \cup \{\seed\}) - \Phi(\seedSetprime)$.
	
	Therefore, the lemma is proved.
\end{proof}
\myparagraph{Drawback}
The greedy algorithm has one limitation. The incremental influence score for every unscanned edge will be calculated in each iteration (line \ref{algo_g-while-for-compute}), which is expensive and not desirable. 

Therefore, we propose two strategies by defining the upper bound of the remaining edges which are not added into \seedSet. 

\myparagraph{UB1} 
Such ``upper bound'' is defined as the aggregated influenced value which each edge can impact at most.

\myparagraph{UB2} 
Interestingly, the upper bound can be incrementally refined in the search process to become increasingly tighter.
Here, we define a novel upper bound for pruning unpromising edges effectively.
Different from the strategy used in UB1, we maintain the maximal marginal
gain value each edge can generate in order to get a tighter upper bound.


\subsection{DP-based Algorithm}
\input{alg-d.tex}
We propose a new algorithm for mining the \resultNum seed edges, namely \partitionlongname. The basic idea is to exploit the graph struture property of road network. Intuitively, a parition is a densely connected subset of vertices and edges that are only sparsely linked to the remaining road network. 

The partition structure is a salient property of road network: Individuals within a partition have frequent contact and thus are more likely to influence each other. In contrast, individuals across partitions have much less contact with each other and thus are less likely to influence each other. Such property suggests that it might be a good approximation to choose influential edges within partitions instead of the whole road network.
Therefore, our \partitionlongname has two phases: \textit{partition} phase and \textit{dp-based selection} phase, which are demonstrated as follows.

\myparagraph{Partition Phase}
%\hui{to do...}
%\hui{I don't think the partition phase in this step will influence the selection algorithm itself in the next step. But a good partition should influence the efficiency greatly, which I still need to explore. Note that, there should have a lot of graph partitions which are only based on the intrinsic nodes and edges, while I think we should also incorporate the diffusion information, like the diffusion probability \diffusePro.}
%There are some options to do the partition: (1) \textbf{MinCut.} We can divide the whole road network based on the traffic volume values of edges in the road network by using the k-way partition \cite{karypis1998fast}, then obtain the partitions by seperating along the cut edges. (2) \textbf{EdgeSim. }
We consider that two edges are similar and can be assigned into one partition if they share more influenced edges. Formally, we define the edge similarity in Definition \ref{def-overlap} as follows:
\begin{definition}
	\label{def-overlap}
	\textit{Edge Similarity. }Given two edges $e_1$ and $e_2$, the overlap distance of these two edges is defined as:
	\begin{equation}
	sim(e_1, e_2) = \frac{|I(e_1)\cap I(e_2)|}{|I(e_1)\cup I(e_2)|}
	\end{equation}
	where $I(\edge)$ is denoted as a set of influenced edges which are impacted by a certain edge \edge during the traffic diffusion.
\end{definition}
To partition the edges into $M$ partitions based on the edge similarity, we adopt the k-means clustering method such that the edges in one partition can influence similar edges. Specifically, we randomly choose $M$ edges as the initial centers of $M$ partitions, then assign the remaining edges into the partition based on the overlap distance with the center edge. In the next iteration, we choose the edge with the maximal influence value as the center edge, and then repeat the previous step until the center edges will not change (or we can give a certain iteration parameter in case the k-means converges too slow). 


\myparagraph{DP-based Selection Phase}
After the \textit{partition phase}, the road network is divided into \partitionNum partitions. Thus one core challenge is how to choose which partitions to find the \resultNum seed edges.
To mine the $k$-th ($1 \leq k \leq \resultNum$) seed edge, we need to choose the partition that will yield the largest increase of influence traffic flow among all the partitions. Then a straightforward solution is to mine top-\resultNum influential
nodes in each partition and then aggregate them to get the
top-\resultNum nodes. This is not desirable as it wastes some computations.
Thus we propose a dynamic programming algorithm to select which partition to find the $k$-th seed edge. 

Given a set of road network partitions $\{P_1, P_2, ..., P_\partitionNum\}$ (line \ref{algo_p-init}), we first initialize an empty seed set \seedSet, an influence score matrix $\weightmatrix[\cdot][\cdot]$, and an indicator matrix $b[\cdot][\cdot]$. For example, $\weightmatrix[m][k]$ (mentioned in line \ref{algo_p-for-for-weight}) refers to the influence score of current found $k$ seed edges from the first $m$ partitions. $b[m][k]$ denotes the partition id where the $k$-th seed edge resides in. Note that, $b[m][k] \leq m$. 

Then a two-loop is executed as follows: for the $k$-th seed edge (line \ref{algo_p-for-start}), we traverse each partition (line \ref{algo_p-for-for-start}) and compute the largest incremental influence score after inserting a possible edge from $P_m$ into \seedSet (line \ref{algo_p-for-for-weightdiff}). After that, we obtain $\weightmatrix[m][k]$ in line \ref{algo_p-for-for-weight}: if the influence score of mining the $k$-th seed edge in the first $m$ partitions is smaller than that in the $m$-th partition $P_m$, then we detect the $k$-th seed edge in $P_m$. Otherwise, we retain the result state $\weightmatrix[m-1][k]$ and find it in the former $m-1$ partitions.
After that, we update the located partition id of the $k$-th seed edge into $b[m][k]$ (lines \ref{algo_p-for-for-if-start}-\ref{algo_p-for-for-if-end}).
At last, the final partition id of $k$-th seed edge is obtained (line \ref{algo_p-for-get}) and we can easily get the selected $k$-th seed edge (line \ref{algo_p-for-maxedge}). 
 


\iffalse
\subsection{Selection Algorithm} 
The motivation of the following method is that: we aim to improve the efficiency and pinpoint the seed edge in each $i$-th iteration. If we find the upper bound of the marginal gain for a partition is smaller than the current found local marginal gain, then this partition can 副be safely pruned to reduce unnecessary actual marginal gain computations. The detail can be found in Algorithm \ref{alg-4}.
\input{alg-p.tex}


\subsection{Some other possible solutions}
There are some other seed selection algorithms for crawling problem in search engine. A typical crawler maintains a list of unvisited URLs
called \textit{frontier}, which is initialized with seed URLs. In each
crawling loop, the crawler picks a URL from the frontier,
fetches the corresponding page, parses the retrieved page
to extract URLs, and adds unvisited URLs to the frontier. Given a currently known portion of the web and the desired number
of seeds \resultNum日, to select seeds so that as many as possible new
good pages will get crawled, and as many as possible currently crawled good pages will be retained. 
\fi





==> tbl-exp.tex <==
\begin{table*}[h]
	\scriptsize 
	\centering
	\renewcommand{\arraystretch}{1.2}
	\caption{Experimental results on different parameters.}
	\label{tbl-exp}
	\begin{tabular}{cccccccc|ccc|ccc}
		\hline
		\multicolumn{8}{c|}{Parameters} & \multicolumn{3}{c|}{Runtime (seconds)} & \multicolumn{3}{c}{$\Phi(S)$} \\ 
		Dataset	&	Period	&\resultNum     & \flowPara    & $w $	& $W$  & $\tau$ & $M$	&\se      & \gr	& \pb	&\se       & \gr	& \pb        \\ \hline
		\chengdu	&	18pm-19pm		&50	&	1&	20&	3600	&9	&50	&126.46		&49.96	&58.338	&447	&485	&478	\\
		%se: 29.876666 46.736496 11.103970 67.791725
		%gr: 23.103298 38.125245 18.633195 1.191047
		%dp: 22.681167 37.315720 18.016265 40.986349
		\chengdu	&	18pm-19pm		&50	&	5&	20&	3600	&9	&50	&78.621	&44.016	&52.371	&270	&275	&275	\\
		\xian	&	18pm-19pm		&50	&	1&	20&	3600	&2	&50	&70.910	&44.743	&67.871	&414	&414	&414	\\
		\xian	&	18pm-19pm		&50	&	4&	20&	3600	&2	&50	&60.066	&46.264	&56.161	&260	&261	&261	\\
		\porto	&	18am-19am		&50	&	1&	20&	3600	&15	&100	&3598.38		&2821.32	&2875.86	&139	&166	&166	\\
		%gr: 1509.37 2669.5 122.31 4.91
		%dp: 1599.5 2581.81 131.33 136.29
		
		\chengdu(small)	&	18pm-19pm		&50	&	1&	20&	3600	&9	&50	&108.947	&41.638	&50.212	&231	&256	&256	\\
		
		\hline		
	\end{tabular}
\end{table*}



==> tbl-influ.tex <==
\begin{table}[h]
	\small
	\renewcommand{\arraystretch}{1.2}
	\caption{An example of traffic diffusion for one spread time window} 
	\label{tbl-diffuse}
	\vspace{-1ex} 
	\centering  
	\subtable[The initial traffic volume $f^0(e)$.]{ 
		%\vspace{1ex}  
		\begin{tabular}{cc|cc}  \hline
			\edge	&	$f^0(e)$	&	\edge	&	$f^0(e)$   \\	\hline
			$e_{1,2}$	&	20	&	$e_{4,5}$	  &	18	\\
			$e_{2,3}$	&	40	  &	  $e_{5,6}$	  &	 36	\\	
			$e_{3,4}$	&	10	&	$e_{6,7}$	&	20	\\	
			$e_{3,6}$	&	24	  &	  $e_{7,8}$	  &	  40	\\	
			$e_{4,2}$	&	16	  &	 $e_{8,5}$	  &	30	\\	\hline
		\end{tabular}  
		\label{tbl-diffuse-one}  
	}  
	\hspace{5ex} 
	\subtable[The traffic volume $f(e)$ after the $1^{st}$ spread time window.]{    
		\vspace{1ex}       
		\begin{tabular}{cc|cc}	\hline
			\edge	&	$f(e)$	&	\edge	&	$f(e)$   \\	\hline
			$e_{1,2}$	&	10	&	$e_{4,5}$	  &	12	\\
			$e_{2,3}$	&	38	  &	  $e_{5,6}$	  &	 42	\\	
			$e_{3,4}$	&	11&	$e_{6,7}$	&	40	\\	
			$e_{3,6}$	&	26	  &	  $e_{7,8}$	  &	  30	\\	
			$e_{4,2}$	&	10	  &		$e_{8,5}$	  &	35	\\	\hline
		\end{tabular}    
		\label{tbl-diffuse-two}  
	}  
\end{table}  

\iffalse
\hspace{5ex} 
\subtable[The traffic volume $f(e)$ after the $2^{nd}$ spread time window.]{    
	\vspace{1ex}       
	\begin{tabular}{cc|cc}	\hline
		\edge	&	$f(e)$	&	\edge	&	$f(e)$   \\	\hline
		$e_{1,2}$	&	10	&	$e_{4,5}$	  &	12	\\
		$e_{2,3}$	&	38	  &	  $e_{5,6}$	  &	 42	\\	
		$e_{3,4}$	&	9.5	&	$e_{6,7}$	&	40	\\	
		$e_{3,6}$	&	22.5	  &	  $e_{7,8}$	  &	  30	\\	
		$e_{4,2}$	&	10	  &		$e_{8,5}$	  &	35	\\	\hline
	\end{tabular}    
	\label{tbl-diffuse-three}  
}  
\fi
